Group analysis of three dimensional Euler equations of gas dynamics

In this paper, the equations governing the unsteady flow of a perfect polytropic gas in three space dimensions are considered. The basic similarity reductions for this system are performed. Reduced equations and exact solutions associated with the symmetries are obtained. This results is used to give the invariance of system up to Galilean motions of space-times $\RR^4$. Then, an optimal system of one-dimensional sub-algebras for symmetry algebra of this system is given.

==> BJGA-MOD.TEX <==
\input bjga.sty %BJGA
\header{1}{10}{Ion Doru Albu, Mihaela Neam\c {t}u and Dumitru Opri\c {s}}
    {The dynamical rigid body with memory}
    {The dynamical rigid body with memory}
%===================================================================
\def\ds{\displaystyle}
\def\ov{\overline}
\newtheorem{proposition}{Proposition}[section]
%===================================================================
\babs
In the present paper we describe the
dynamics of the revised rigid body, the dynamics of the rigid body
with distributed delays and the dynamics of the fractional rigid
body. We analyze the stationary states for given values of the
rigid body's parameters.
\eabs\msc 26A33, 53C63,58A05, 58A40.
\kwd rigid body, revised rigid body, distributed delay, fractional derivative.

\section{Introduction}
\par In mechanical problems, the dynamics of the rigid body has an
important role. In many papers M. Puta analyzed the dynamics of
the rigid body with control and he obtained important results.
\par Recently, the dynamics of revised rigid body, the dynamics of
the rigid body with distributed delay and the dynamics of the
rigid body with fractional derivative have been studied. The last
two aspects represent the dynamics of the rigid body with memory.
\par Our paper studies the dynamics of the revised rigid body
obtained by a metriplectic structure which is canonically
associated. We define the dynamics of the rigid body with
distributed delays. For the Euler-Poincare dynamics of the rigid
body we analyze the linearized system in an equilibrium point. We
obtain the the existence conditions for the Hopf bifurcation with
respect to the parameter of the repartition density which defines
the distributed delay. Also, we define the fractional rigid body
dynamics using the Caputo fractional derivative.

\section{The revised differential equations for the rigid body}

The differential equations for the rigid body in $ {\mathbb R}^3$
are described by a 2-antisymmetric tensor field P and the
Hamiltonian function h given by:
\begin{equation}
P(x)=(P^{ij}(x))=\left (\begin{array}{ccc}0&x^3&-x^2\\
-x^3&0&x^1\\x^2&-x^1&0\label{1}
\end{array}\right ), \quad
h=\ds\frac{1}{2}(a_1(x^1)^2+a_2(x^2)^2+a_3(x^3)^2),
\end{equation} where $(x^1,x^2,x^3)^T\in {\mathbb R}^3$, $a_i\in{\mathbb
R_+}$, $i=1,2,3$, $a_1>a_2>a_3$. These differential equations are:
\begin{equation}
\dot x(t)=P(x(t))\nabla_xh(x(t)),\label{2}
\end{equation} where $\dot x(t)=(\dot x^1(t), \dot x^2(t), \dot
x^3(t))^T$ and $\nabla_xh$ is the gradient of $h$ with respect to
the canonical metric on ${\mathbb R}^3$. The differential
equations (\ref{2}) have been studied by M. Puta in \cite{8b}.
\par Let ${\mathbb R}^3$ be the space interpreted as the space of body
angular velocities $\Omega$ equipped with the cross product as the
Lie bracket. On this space, we consider the standard Lagrangian
 kinetic energy $L(\Omega)=\ds\frac{1}{2}I\cdot \Omega$, where
$I=diag(I_1,I_2,I_3)$ is the moment of inertial tensor, so that
the general Euler-Poincare equations become the standard rigid
body equations for a freely spinning rigid body:

\begin{equation} I\dot \Omega=(I\cdot \Omega)\times\Omega.\label{3}
\end{equation}

If $M=I\cdot\Omega$ is the angular momentum, then, (\ref{3}) is:

\begin{equation}\dot M=M\times \Omega.\label{4}
\end{equation}

\par  If $M=(I_1x(t), I_2y(t),I_3z(t))^T$,
$\Omega=(x(t),y(t),z(t))^T$ from (\ref{4}) results:
\begin{equation}
\dot x(t)=\ds\frac{I_2-I_3}{I_1}y(t)z(t),\quad \dot
y(t)=\ds\frac{I_3-I_1}{I_2}x(t)z(t),\quad  \dot
z(t)=\ds\frac{I_1-I_2}{I_3}x(t)z(t),\label{5}
\end{equation}
 with $I_1>I_2>I_3$.
The differential equations (\ref{5}) have been studied by M. Puta
in \cite{8b}. The revised differential equations for the rigid
body given by (\ref{2}) have been studied in \cite{5b}. They are
described by P, h and the tensor fields $g=(g^{ij}(x))$, where P
and h are given by (\ref{1}) and g is defined by
$g(x)=(g^{ij}(x)),$
\begin{equation*}
g^{ij}(x)=\ds\frac{\partial h(x)}{\partial x^i}\ds\frac{\partial
h(x)}{\partial x^j}, i\neq j, g^{ij}(x)=-\sum_{k=1,k\neq
i}^3(\ds\frac{\partial h(x)}{\partial x^k})^2, i=1,2,3
\end{equation*} and the Casimir function of the Poisson structure P is:
\begin{equation*}
c(x)=\ds\frac{1}{2}((x^1)^2+(x^2)^2+(x^3)^3).
\end{equation*}

The structure $({\mathbb R}^3,P,g,h,c)$ is called a metriplectic
manifold of second kind. The revised differential system
associated to (\ref{2}) is given by:
\begin{equation}
\dot x(t)=P(x)\nabla_xh(x)+g(x)\nabla_xc(x).\label{6}
\end{equation}

\begin{proposition}(i) The differential equations (\ref{2}) are given
by:

\begin{equation}\dot x^1(t)\!=\!(a_2\!-\!a_3)x^2(t)x^3(t), \dot
x^2(t)\!=\!(a_3\!-\!a_1)x^1(t)x^3(t), \dot
x^3(t)\!=\!(a_1\!-\!a_2)x^1(t)x^2(t);\label{7}
\end{equation}
(ii) The differential equations (\ref{6}) are given by:
\begin{equation}
\begin{split}
\dot x^1(t)\!=\!(a_2\!-\!a_3)x^2(t)x^3(t)\!
+\!a_2(a_1\!-\!a_2)x^1(t)(x^2(t))^2\!+\!a_3(a_1\!-\!a_3)x^1(t)(x^3(t))^2\\
\dot x^2(t)\!=\!(a_3\!-\!a_1)x^1(t)x^3(t)\!
+\!a_3(a_2\!-\!a_3)x^2(t)(x^3(t))^2\!+\!a_1(a_2\!-\!a_1)x^2(t)(x^1(t))^2\\
\dot x^3(t)\!=\!(a_1\!-\!a_2)x^1(t)x^2(t)\!
+\!a_1(a_3\!-\!a_1)x^3(t)(x^1(t))^2\!+\!a_2(a_3\!-\!a_2)x^3(t)(x^2(t))^2.\label{8}
\end{split}
\end{equation}
\end{proposition}
The equilibrium points of the system (\ref{7}) are studied in [8]
and the equilibrium points of the system (\ref{8}) in \cite{5b}.

\section{The differential system with distributed delay for the
rigid body}

\hspace{0.6cm} We consider the space ${\mathbb R}^3$, the product
${\mathbb R}^3\times{\mathbb R}^3=\{(\tilde x,x),\tilde
x\in{\mathbb R}^3, x\in{\mathbb R}^3\}$ and the canonical
projections $\pi_i:{\mathbb R}^3\times{\mathbb R}^3\rightarrow
{\mathbb R}^3$, $i=1,2$. A vector field $X\in{\cal X}({\mathbb
R}^3\times {\mathbb R}^3)$ satisfying the condition
$X(\pi^*_1f)=0$, for any $f\in C^\infty({\mathbb R}^3)$ is given
by:
\begin{equation*}
X(\tilde x,x)=\sum_{i=1}^3X_i(\tilde
x,x)\ds\frac{\partial}{\partial x_i}.
\end{equation*}

The differential system associated to $X$ is given by:
\begin{equation*}
\dot x^i(t)=X^i(\tilde x(t),x(t)), i=1,2,3.
\end{equation*}
A differential system with distributed delay is a differential
system associates to a vector field $X\in{\cal X}({\mathbb
R}^3\times {\mathbb R}^3)$ for which $X(\pi^*_1f)=0$, for any
$f\in C^\infty({\mathbb R}^3)$ and it is given by (1), where
$\tilde x(t)$ is:
\begin{equation*}
\tilde x(t)=\int_0^k k(s)x(t-s)ds,
\end{equation*} where $k(s)$ is a density of repartition.
In what follows, we will consider the case of the following
densities of repartition:

(i) the uniform density with:
\begin{equation*}
k_\tau(s)=\left\{\begin{array}{lll} 0,& 0\leq s\leq a\\
\ds\frac{1}{\tau}, & a\leq s\leq a+\tau\\
0, &s>a+\tau\end{array},\right.
\end{equation*} where $a>0$, $\tau>0$ are given numbers;

(ii) the exponential density, with $k_\alpha(s)=\alpha e^{-\alpha
s}, \quad \alpha>0;$

(iii) the Erlang density, with $k_\alpha(s)=\alpha^2se^{-\alpha
s}, \quad \alpha>0$;

(iv) the Dirac density, with $k_\tau(s)=\delta(s-\tau), \quad
\tau>0$.

The initial condition is: $ x(s)=\varphi(s), \quad
s\in(-\infty,0],$ \\ with $\varphi:(-\infty,0]\rightarrow{\mathbb
R}^3$ a smooth map. Some systems of differential equations with
distributed delay in ${\mathbb R}^3$ were studied in \cite{1b},
\cite{2b}. For such a system, we consider relevant the geometric
properties of the vector field which defines the system, for
example first integrals (constants of the motion), Morse
functions, almost metriplectic structure, etc. The differential
equations with distributed delay for rigid body are
ge\-ne\-ra\-ted by a 2-antisymmetric tensor field P on ${\mathbb
R}^3\times{\mathbb R}^3$ that satisfies the following relations:
$P(\pi^*_1f_1,\pi^*_2f_2)=0, P(\pi^*_2f_1,\pi^*_2f_2)=0,$  for all
$f_1$, $f_2$ $\in C^\infty({\mathbb R}^3)$ and $h\in
C^\infty({\mathbb R}^3\times{\mathbb R}^3)$. The differential
equation is given by:
\begin{equation}
\dot x=P(\tilde x,x)\nabla_xh(\tilde x,x).\label{9}
\end{equation}

Let $P(\tilde x,x)$ be the tensor field  with the components given
by:
\begin{equation}
(P^{ij}(x,x))=\left(\begin{array}{ccc} 0 & x^3 &-\tilde
x{}^2\\
-x^3 & 0 & x^1\\
\tilde x{}^2 & -x^1 & 0\end{array}\right)\label{10}
\end{equation} and
\begin{equation}
h\left(\tilde x, x\right)=a_1\tilde x{}^1x^1+a_2\tilde x{}^2
x^2+a_3\tilde x{}^3 x^3.\label{11}
\end{equation}

The differential equations (\ref{9}) are:
\begin{equation*}
\begin{array}{l}
\vspace{0.1cm} \dot x{}^1(t)=a_2 \tilde x^2(t)x^3(t)-a_3 \tilde
x^2(t)\tilde x^3(t),\\
\vspace{0.1cm} \dot x{}^2(t)=a_3 x^1(t)\tilde x^3(t)-a_1
\tilde x^1(t)x^3(t),\\
\dot x{}^3(t)=a_1 \tilde x^1(t)\tilde x^2(t)-a_2 x^1(t)\tilde
x^2(t).\end{array}
\end{equation*}

The differential system:
\begin{equation}
\dot x=P(\tilde x,x)\nabla_xh(\tilde x,x)+g(\tilde
x,x)\nabla_xc(\tilde x,x),\label{12}
\end{equation} where the components of
$g(\tilde x,x)$ are:
\begin{equation}
g^{ij}(x)=\ds\frac{\partial h(x,\tilde{x})}{\partial
x^i}\ds\frac{\partial c(x,\tilde{x})}{\partial x^j}, i\neq j,
g^{ii}(x)=-\sum_{k=1,k\neq i}^3\ds\frac{\partial
h(x,\tilde{x})}{\partial x^k}\ds\frac{\partial
c(x,\tilde{x})}{\partial x^k}, i=1,2,3\label{13}
\end{equation} is called the revised differential system with
distributed delay associated to the differential system (\ref{9}).

From (\ref{10}), (\ref{11}), (\ref{13}) and $c(\tilde
x,x)=\frac{1}{2}(x^1)^2+x^2\tilde x^2+\frac{1}{2}(x^3)^2$ results:
\begin{equation*}
(g^{ij})\!=\!\left(\begin{array}{cccc} \vspace{0.1cm}
 -a_2^2x^2\tilde x{}^2-a_3x^3\tilde
x{}^3 & a_1a_2\tilde x{}^1 x^2 & a_1 a_3\tilde x{}^1 x^3\\
\vspace{0.1cm} a_1a_2\tilde x{}^1x^2 & -a_1^2x^1\tilde
x{}^1-a_3x^3\tilde
x{}^3 & a_2a_3\tilde x{}^2x^3\\
a_1a_3\tilde x{}^1x^2 & a_2a_3\tilde x{}^2x^3 & -a_1^2x^1\tilde
x{}^1-a_2^2x^2\tilde x{}^2\end{array}\right).
\end{equation*}

The differential system (\ref{12}) is given by:
\begin{equation}
\begin{array}{lll}
\vspace{0.1cm} \dot
x{}^1(t)&=&a_2\tilde x^2(t)x^3(t)-a_3\tilde x^2(t)\tilde x^3(t)+a_1a_2\tilde x^1(t)(x^2(t))^2,\\
\dot x{}^2(t)&=& a_3x^1(t)\tilde x^3(t)-a_1\tilde x^1(t)x^3(t)-a_1^2x^1(t)\tilde x^1(t)x^2(t)-a_3^2x^2(t)x^3(t)\tilde x^3(t),\\
\dot x{}^3(t)&=& a_1\tilde x^1(t)x^2(t)-a_2 x^1(t)\tilde
x^2(t)+a_2a_3\tilde x^2(t)x^2x^3.\end{array}\label{14}
\end{equation}

For the Dirac distribution, system (\ref{14}) was analyzed in
\cite{6b}. The other types of densities will be analyzed in our
future papers.

The Euler-Poincare equation for the free rigid body with
distributed delay is defined by:
\begin{equation*}
\dot M=M\times\Omega+\alpha M\times(\tilde M\times\tilde\Omega)
\end{equation*} where $M=(I_1x(t),I_2y(t),I_3z(t))^T$,
$\Omega=(x(t),y(t),z(t))^T$, $\tilde \Omega=(\tilde x(t),\tilde
y(t), \tilde z(t))^T$, $\tilde M=I\tilde\Omega$, $I_1>0$, $I_2>0$,
$I_3>0$ and $\alpha\in{\mathbb R}$.

The equilibrium points of our system are
$\Omega_1=(\frac{m}{I_1},0,0)^T$,
$\Omega_2=(0,\frac{m}{I_2},0)^T$,
$\Omega_3=(0,0,\frac{m}{I_3})^T$, $m\in{\mathbb R}^*$.

\begin{proposition} The equilibrium point $\Omega_1$ has the
following behavior:

(i) The corresponding linear system is given by:
\begin{equation*}
\dot U(t)=AU(t)+\alpha B\tilde U(t)
\end{equation*} where $U(t)=(u^1(t),u^2(t),u^3(t))^T$ and
\begin{equation*}
A=\left(\begin{array}{ccc}0& 0& 0\\
0& 0& \frac{I_3-I_1}{I_1I_2}m\\
0& \frac{I_1-I_2}{I_1I_3}m& 0
\end{array}\right ), B=\left(\begin{array}{ccc}0& 0& 0\\
0& \frac{I_2-I_1}{I_1I_2}m^2& 0\\
0& 0& \frac{I_3-I_1}{I_1I_3}m^2
\end{array}\right );
\end{equation*}

(ii) The characteristic equation is:
\begin{equation*}
\begin{split}
&\lambda[\lambda^2-\frac{\alpha
m^2}{I_1}(\frac{I_2-I_1}{I_2}+\frac{I_3-I_1}{I_3})\lambda
k^{(1)}(\lambda)+\frac{\alpha^2m^4}{I_1^2I_2I_3}(I_2-I_1)(I_3-I_1)k^{(1)}(\lambda)^2-\\
&\frac{(I_1-I_2)(I_3-I_1)}{I_1^2I_2I_3}m^2]=0;
\end{split}
\end{equation*}

(iii) On the tangent space at $\Omega_1$ to the sphere of radius
$m^2$ the linear operator given by the linearized vector field has
the characteristic equation:

\begin{equation*}
\begin{split}
&\lambda^2-\frac{\alpha
m^2}{I_1}(\frac{I_2-I_1}{I_2}+\frac{I_3-I_1}{I_3})\lambda
k^{(1)}(\lambda)+\frac{\alpha^2m^4}{I_1^2I_2I_3}(I_2-I_1)(I_3-I_1)k^{(1)}(\lambda)^2-\\
&\frac{(I_1-I_2)(I_3-I_1)}{I_1^2I_2I_3}m^2]=0;
\end{split}
\end{equation*}

(iv) If $I_1>I_2$, $I_1>I_3$ and
$k^{(1)}(\lambda)=e^{-\tau\lambda}$, $\tau>0$, for
$0\leq\tau<\tau_c$, where
\begin{equation*}
\tau_c=\ds\frac{I_1(I_3(I_1-I_2)+I_2(I_1-I_3))}{3|\alpha|m^2(I_1-I_2)(I_1-I_3)},
\end{equation*} then the equilibrium point $\Omega_1$ is
asymptotically stable.
\end{proposition}

The analysis of the equilibrium point $\Omega_1$ for the Dirac
density is given in \cite{1b}.

\section{Fractional differential systems for the rigid body}

\hspace{0.6cm} Generally speaking, the fractional derivative,
Riemann-Liouville fractional derivative and Caputo's fractional
derivative are mostly used. In the present paper we discuss the
Caputo derivative:
\begin{equation*}
D^\alpha_tx(t)=I^{m-\alpha}(\ds\frac{d}{dt})^mx(t), \quad
\alpha>0,
\end{equation*} where $m-1<\alpha\leq m$,
$(\ds\frac{d}{dt})^m=\ds\frac{d}{dt}\circ...\circ\ds\frac{d}{dt}$,
$I^\beta$ is the $\beta$th order Riemann-Liouville integral
operator, which is expressed as follows:
\begin{equation*}
I^\beta
x(t)=\ds\frac{1}{\Gamma(\beta)}\int_0^t(t-s)^{\beta-1}x(s)ds,
\quad \beta>0.
\end{equation*}

In this paper, we suppose that $\alpha\in(0,1)$.

Examples of the fractional differential systems are: the
fractional order of Chua's system, the fractional order of
Rossler's system and the fractional Duffing oscillator. The
geometrical and mechanical interpretation of the fractional
derivative is given in \cite{7b}. The geometry of fractional
osculator bundle of higher order was made in \cite{3b} using the
fractional differential forms defined in \cite{4b}.


Let ${\cal X}^\alpha({\mathbb R}^3)$ be the module of the
fractional vector fields generated by the operators
$\{D^\alpha_{x^i}, i=1,2,3\}$ and the module ${\cal D}({\mathbb
R}^3)$ generated by 1-forms $\{d(x^i)^\alpha, i=1,2,3\}$. The
fractional exterior derivative $d^\alpha:C^\infty({\mathbb
R}^3)\rightarrow{\cal D}({\mathbb R}^3)$ is defined by:
\begin{equation*}
d^\alpha(f)=d(x^i)^\alpha D^\alpha_{x^i}(f).
\end{equation*}

Let ${\mathop{{P}}\limits^{\alpha}}\in{\cal
X}^\alpha(\mathbb{R}^{3})\times {\cal X}^\alpha(\mathbb{R}^{3})$
be a fractional 2-skew-symmetric tensor field and $d^\alpha f$,
$d^\alpha g\in{\cal D}({\mathbb R}^3)$. The bilinear map
$[\cdot,\cdot]^\alpha:C^\infty(\mathbb{R}^{3})\times
C^\infty(\mathbb{R}^{3})\rightarrow C^\infty(\mathbb{R}^{3})$
defined by:
\begin{equation}
[f,g]^\alpha={\mathop{{P}}\limits^{\alpha}}(d^\alpha f, d^\alpha
g), \forall f,g\in C^\infty (\mathbb{R}^{3})\label{21}
\end{equation} is called the fractional Leibniz bracket.

If
${\mathop{{P}}\limits^{\alpha}}={\mathop{{P}}\limits^{\alpha}}{}^{ij}D^\alpha_{x^i}\otimes
D^\alpha_{x^j}$ then from (\ref{21}) it follows that:
\begin{equation*}
[f,g]^\alpha={\mathop{{P}}\limits^{\alpha}}{}^{ij}D^\alpha_{x^i}fD^\alpha_{x^j}g.
\end{equation*}

From the properties of the fractional Caputo, results:
\begin{equation*}
\begin{split}
&[fh,g]^\alpha=\sum\limits^\infty_{k=0}\left(\begin{array}{c}\alpha\\k\end{array}\right){\mathop{{P}}\limits^{\alpha}}{}^{ij}
(D^{\alpha-k}_{x^i}f)(D^{\alpha}_{x^j}g)\left
(\frac{\partial}{\partial x^i}\right)^kh\\
&[f,gh]^\alpha=\sum\limits^\infty_{k=0}\left(\begin{array}{c}\alpha\\k\end{array}\right){\mathop{{P}}\limits^{\alpha}}{}^{ij}
(D^{\alpha}_{x^i}f)(D^{\alpha-k}_{x^j}g)\left
(\frac{\partial}{\partial x^i}\right)^kh.
\end{split}
\end{equation*}

If ${\mathop{{P}}\limits^{\alpha}}$ is skew-symmetric we say that
$({\mathbb R}^3,[\cdot,\cdot]^\alpha)$ is a fractional almost
Poisson manifold. If $\alpha\rightarrow 1$ then we obtain the
concepts from \cite{8b}.

For $h\in C^\infty({\mathbb R}^3)$, the fractional almost Poisson
dynamic system is given by:
\begin{equation}
D^\alpha_tx^i(t)=[x^i(t),h(t)]^\alpha, \textrm{where}
[x^i,h]^\alpha={\mathop{{P}}\limits^{\alpha}}{}^{ij}D^\alpha_{x^j}h.\label{22}
\end{equation}

Let ${\mathop{{P}}\limits^{\alpha}}$ be a 2-skew-symmetric
fractional tensor field and ${\mathop{{g}}\limits^{\alpha}}$ a
2-symmetric fractional tensor field on ${\mathbb R}^3$. We define
the bracket $[\cdot,\cdot]^\alpha:C^\infty({\mathbb R}^3)\times
C^\infty({\mathbb R}^3)\rightarrow C^\infty({\mathbb R}^3)$ by:
\begin{equation*}
[f,h]^\alpha={\mathop{{P}}\limits^{\alpha}}(d^\alpha f, d^\alpha
g)+{\mathop{{g}}\limits^{\alpha}}(d^\alpha f, d^\alpha h), \quad
f,h\in C^\infty(\mathbb{R}^{3}).
\end{equation*}

The structure $(M, {\mathop{{P}}\limits^{\alpha}},
{\mathop{{g}}\limits^{\alpha}}, [\cdot,\cdot])$ is called
fractional almost metriplectic manifold. The fractional dynamic
system associated to $h\in C^\infty(\mathbb{R}^{3})$ is
\begin{equation}
D^\alpha_tx^i(t)=[x^i(t),h(t)]^\alpha, \textrm{where}
 [x^i,h]^\alpha={\mathop{{P}}\limits^{\alpha}}{}^{ij}D^\alpha_{x^j}h+
{\mathop{{g}}\limits^{\alpha}}{}^{ij}D^\alpha_{x^j}h.\label{23}
\end{equation}

If we define the bracket
$[\cdot,(\cdot,\cdot)]^\alpha:C^\infty({\mathbb R}^3)\times
C^\infty({\mathbb R}^3)\times C^\infty({\mathbb R}^3)\rightarrow
C^\infty({\mathbb R}^3)$ by:
\begin{equation*}
[f,(h_1,h_2)]^{\alpha}={\mathop{{P}}\limits^{\alpha}}(d^\alpha f,
d^\alpha h_1)+{\mathop{{g}}\limits^{\alpha}}(d^\alpha f, d^\alpha
h_2), \forall f,h_1,h_2\in C^\infty({\mathbb R}^3),
\end{equation*} then, the fractional vector field
${\mathop{{X}}\limits^{\alpha}}{}_{h_1h_2}$ defined by:
\begin{equation*}
{\mathop{{X}}\limits^{\alpha}}{}_{h_1h_2}(f)=[f,(h_1,h_2)]^{\alpha},
\forall f\in C^\infty({\mathbb R}^3)
\end{equation*} is called the fractional almost Leibniz vector
field associated to the functions $h_1$, $h_2\in C^\infty({\mathbb
R}^3)$. \par The fractional almost Leibniz dynamical system is
given by:
\begin{equation*}
D^\alpha_tx^i(t)={\mathop{{P}}\limits^{\alpha}}{}^{ij}D^\alpha_{x^j}h_1+
{\mathop{{g}}\limits^{\alpha}}{}^{ij}D^\alpha_{x^j}h_2.
\end{equation*}

Let ${\mathop{{P}}\limits^{\alpha}}=(P^{ij})$,
${\mathop{{g}}\limits^{\alpha}}=(g^{ij})$ be the fractional
2-tensor fields on ${\mathbb R}^3$ and $h\in C^\infty({\mathbb
R}^3)$ given by:
\begin{equation*}
h=\ds\frac{1}{\Gamma(\alpha+1)}[a_1(x^1)^{\alpha+1}+a_2(x^2)^{\alpha+1}+a_3(x^3)^{\alpha+1}].
\end{equation*}

\begin{proposition} (i) The fractional dynamic system (\ref{22}) is:
\begin{equation}
D^\alpha_tx^1=(a_2-a_3)x^2x^3, D^\alpha_tx^2=(a_3-a_1)x^1x^3,
D^\alpha_tx^3=(a_1-a_2)x^1x^2;\label{24}
\end{equation}

(ii) The fractional dynamic system (\ref{23}) is:
\begin{equation}
\begin{split}
&D^\alpha_tx^1=(a_2-a_3)x^2x^3+a_2(a_1-a_2)x^1(x^2)^2+a_3(a_1-a_3)x^1(x^3)^2\\
&D^\alpha_tx^2=(a_3-a_1)x^1x^3+a_3(a_2-a_3)x^2(x^3)^2+a_1(a_2-a_1)x^2(x^1)^2\\
&D^\alpha_tx^3=(a_1-a_2)x^1x^2+a_1(a_3-a_1)x^3(x^1)^2+a_2(a_3-a_2)x^3(x^2)^2;\label{25}
\end{split}
\end{equation}

(iii) The fractional dynamic systems (\ref{24}) and (\ref{25})
have the equilibrium points $M_1(m,0,0)$, $M_2(0,m,0)$,
$M_3(0,0,m)$, $m\in{\mathbb R}^*$;

(iv) The characteristic equations for (\ref{24}) are:

in $M_1(m,0,0)$: $
\lambda^\alpha(\lambda^{2\alpha}+(a_1-a_3)(a_1-a_2)m^2)=0,$

in $M_2(0,m,0)$:
$\lambda^\alpha(\lambda^{2\alpha}-(a_1-a_2)(a_2-a_3)m^2)=0,$

in $M_3(0,0,m)$:
$\lambda^\alpha(\lambda^{2\alpha}+(a_1-a_3)(a_2-a_3)m^2)=0;$ (v)
The characteristic equations in $M_1(m,0,0), \, M_2(0,m,0), \,
M_3(0,0,m)$ for (\ref{25}) are:
$$\lambda^\alpha(\lambda^{2\alpha}-a_1(a_2+a_3-2a_1)m^2\lambda^\alpha+(a_1-a_3)(a_1-a_2)m^2(a_1^2m^2+1))=0,$$
$$\lambda^\alpha(\lambda^{2\alpha}-a_2(a_1+a_3-2a_2)m^2\lambda^\alpha-(a_1-a_2)(a_2-a_3)m^2(a_2^2m^2+1))=0,$$
$$\lambda^\alpha(\lambda^{2\alpha}-a_3(a_1+a_2-2a_3)m^2\lambda^\alpha+(a_1-a_3)(a_2-a_3)m^2(a_3^2m^2+1))=0;$$
\end{proposition}

The above findings allow the analysis of the equilibrium points
with respect to the parameters of the characteristic equations.

Equations (\ref{24}) are called the fractional equations of the
rigid body and equations (\ref{25}) are called revised fractional
equations of the rigid body. If $\alpha\rightarrow 1$, the results
from Proposition 4.2 lead to results from \cite{8b}.

\par For $a_{1}:=3, \,
a_{2}:=2, \, a_{3}:=1, \, \alpha=1$ the dynamics
$(x^1(t),x^2(t),x^3(t))$ of (\ref{24}) is given in figure Fig.1
and for $\alpha=0.82$ in figure Fig.2. The numerical algorithm
used is Adam-Moulton-Bashford.

%\begin{center}\begin{tabular}{ccc}
%\includegraphics[width=6cm]{p-al1.eps} & &
%\includegraphics[width=6cm]{p-al2.eps}
%\end{tabular}
%\end{center}

\section{Conclusions}
\hspace{0.6cm} In the present paper we present the dynamics of the
rigid body with memory. The memory was described by the variables
with distributed delay and by the Caputo fractional derivative.

\bebi
\bibitem{1b} {I.D. Albu, M. Neamtu and D. Opris}, {\em Dissipative mechanical systems with
delay}, Tensor N.S. 67 (2006), 1-27.
\bibitem{2b} {I.D. Albu, D.Opris}, {\em Leibnitz dynamics with time delay}, arXiv.math/0508225.
\bibitem{3b} {I.D. Albu, M. Neamtu and D. Opris}, {\em The geometry of fractional osculator bundle of higher order and applications}, International Conference on Differential Geometry Lagrange and Hamilton Spaces, Iasi, September, 3-8, 2007, Scintific Annals of
"Al. I. Cuza" University, Mathematics, LIII (2007):21-32,
arXiv:0709.2000v1, math.DG, 2007.
\bibitem{4b}  {W. Deng, C. Li and J. L$\ddot{u}$}, {\em Stability analysis of linear differential systems with multiple time delay}, Nonlinear Syn. 48 (2007), 409-416.
\bibitem{5b}  {D. Fish}, {\em Dissipative perturbations of 3D Hamiltonian
systems}, arXiv:math/0506047v1, 2005.
\bibitem{6b}  {M. Neamtu, D. Opris and M. Popescu}, {\em Hopf Bifurcation for the Rigid
Body with Time Delay}, Proceedings of the 5th conference of
Balkan Society of Geometers, Geometry Balkan Press, Bucharest 2006, 83-92.
\bibitem{7b}  {I. Podlubny}, {\em Geometrical and physical interpretation of
fractional integration and fractional differentiation},
Fractional Calculus and Applied Analysis 5, 4 (2002), 367-386.
\bibitem{8b}  {M. Puta}, {\em Hamiltonian systems and geometric
quantisation}, Mathematics and Applications, Vol. 260, Kluwer
Academic Publishers 2004.
\eebi
\auas
Ion Doru Albu and Dumitru Opri\c{s}\\
Department of Mathematics, Faculty of Mathematics, \\
West University of Timi\c{s}oara,\\
4 Bd. V. Parvan, 300223, Timi\c soara, Romania.\\
E-mail: albud@math.uvt.ro, opris@math.uvt.ro\\\\
Mihaela Neam\c{t}u \\
Department of Economic Informatics and Statistics,\\
Faculty of Economics, West University of Timi\c{s}oara,\\
16A Pestalozzi St., 300115, Timi\c{s}oara, Romania.\\
E-mail:mihaela.neamtu@fse.uvt.ro
\end{document}


==> Ma_038_Bal.tex <==
\input bjga.sty
\begin{document}
\def\be{\begin{eqnarray}}
\def\ee{\end{eqnarray}}
\def\RR{{\Bbb R}}
\def\Span{\mathrm{Span}}
\title{Group analysis of three dimensional \\ Euler equations of gas dynamics}
\author{Mehdi Nadjafikhah\thanks{Faculty of Mathematics, Iran University
of Science and Technology, Narmak, Tehran, I.R.IRAN. e-mail:
m\_nadjafikhah@iust.ac.ir} }
%
\date{}
%
\maketitle
%
\babs In this paper, the equations governing the unsteady flow of
a perfect polytropic gas in three space dimensions are considered.
The basic similarity reductions for this system are performed.
Reduced equations and exact solutions associated with the
symmetries are obtained. This results is used to give the
invariance of system up to Galilean motions of space-times
$\RR^4$. Then, an optimal system of one-dimensional sub-algebras
for symmetry algebra of this system is given.
%
\eabs\msc 35C05, 76M60.
%
\kwd Euler equations, Lie group of
transformations, Symmetry generators, Similarity solution, optimal
system of Lie sub-algebras.
%
%
\section{Introduction}
%
%
The equations governing the unsteady flow of a perfect polytropic
gas in three space dimensions are
%
\be
%
&&\hspace{-1cm}  \frac{\partial u}{\partial t}+u\frac{\partial
u}{\partial x}+v\frac{\partial u}{\partial y}+w\frac{\partial
u}{\partial z}
+\frac{1}{q}\frac{\partial p}{\partial x}=0,\nonumber \\
%
&&\hspace{-1cm}  \frac{\partial v}{\partial t}+u\frac{\partial
v}{\partial x}+v\frac{\partial v}{\partial y}+w\frac{\partial
v}{\partial z}
+\frac{1}{q}\frac{\partial p}{\partial y}=0,\nonumber \\
%
&&\hspace{-1cm}  \frac{\partial w}{\partial t}+u\frac{\partial
w}{\partial x}+v\frac{\partial w}{\partial y}+w\frac{\partial
w}{\partial z}
+\frac{1}{q}\frac{\partial p}{\partial z}=0,\label{eq:1}\\
%
&&\hspace{-1cm}  \frac{\partial q}{\partial
t}+q\Big(\frac{\partial u}{\partial x}+\frac{\partial v}{\partial
y}+\frac{\partial w}{\partial z}\Big)+u\frac{\partial q}{\partial
x}+v\frac{\partial q}{\partial
y}+w\frac{\partial q}{\partial z}=0,\nonumber \\
%
&&\hspace{-1cm}  \frac{\partial p}{\partial t}+\gamma
p\Big(\frac{\partial u}{\partial x}+\frac{\partial v}{\partial
y}+\frac{\partial w}{\partial z}\Big)+u\frac{\partial p}{\partial
x}+v\frac{\partial p}{\partial y}+w\frac{\partial p}{\partial
z}=0.\nonumber
%
\ee
%
where $t$ is the time and $x$, $y$, $z$ are the space coordinates;
$q(t,x,y,z)$ is the density, $p(t,x,y,z)$ the pressure,
$u(t,x,y,z)$, $v(t,x,y,z)$ and $w(t,x,y,z)$ the velocity
components in the $x$, $y$ and $z$ directions, respectively, and
$\gamma\in\RR$ is the adiabatic index. These equations are called
"{\it three dimensional Euler equations of gas dynamics}"
\cite{SekSha} and section 6.3 of \cite{Ste}.

 In this paper, we consider the equations governing the
unsteady flow of a perfect polytropic gas in three space
dimensions. The basic similarity reductions for this system are
performed. Reduced equations and exact solutions associated with
the symmetries are obtained. We find an optimal system of
one-dimensional sub-algebras for symmetry algebra of this system.

In section 2 we find the full symmetry algebra of system
(\ref{eq:1}). Section 3 is devoted to the group-invariant
solutions to the system. The structure of full symmetry algebra
illustrated in section. The last section deals with a optimal
system of sub-algebras.
%
%
\section{Lie symmetry of the system}
%
%
The classical method for finding symmetry reductions of PDE is the
Lie group method of infinitesimal transformations. To apply the
classical method to (\ref{eq:1}), we consider the one-parameter
Lie group of infinitesimal transformations in $(t,x,y,z,u,v,p,q)$
given by
%
\begin{align} \tilde{t} &= t+s.\xi_1(t,\cdots,q)+O(s^2),\nonumber\\
\tilde{x} &= x+s.\xi_2(t,\cdots,q)+O(s^2), &
\tilde{y} &= y+s.\xi_3(t,\cdots,q)+O(s^2),\nonumber\\
\tilde{z} &= z+s.\xi_4(t,\cdots,q)+O(s^2), &
\tilde{u} &= u+s.\eta_1(t,\cdots,q)+O(s^2),\\
\tilde{v} &= v+s.\eta_2(t,\cdots,q)+O(s^2), &
\tilde{w} &= w+s.\eta_3(t,\cdots,q)+O(s^2),\nonumber\\
\tilde{p} &= p+s.\eta_4(t,\cdots,q)+O(s^2), & \tilde{q} &=
q+s.\eta_5(t,\cdots,q)+O(s^2). \nonumber
\end{align}
%
where $s$ is the group parameter. One requires that this
transformation leaves the sub-manifold $S$ invariant. Let
$$X=\xi_1\,\partial_t+\xi_2\,\partial_x+\xi_3\,\partial_y+\xi_4\,
\partial_z+\eta_1\,\partial_u+\eta_2\,\partial_v+\eta_3\,\partial_w+\eta_4\,\partial_p+\eta_5\,\partial_q$$
 be the corresponding infinitesimal transformation; where
coefficients are real-valued $C^\infty-$functions of
$t,x,y,z,u,v,w,p,q$. The infinitesimal criterion of invariance
(\ref{eq:1}) will thus involve $t,x,y,z,u,v,w,p,q$ and the
derivatives of $u,v,w,p,q$ with respect to $t,x,y,z$, as well as
$\xi_i$, $i=1,2,3,4$, and $\eta_j$, $j=1,2,3,4,5$, and their
partial derivatives. After eliminating any dependencies among the
derivatives of the m's caused by the system itself, we can then
equate the coefficients of the remaining unconstrained partial
derivatives of u to zero. This will result in a large number of
elementary partial differential equations for the coefficient
functions $\xi_i$, $\eta_j$ of the infinitesimal generator, called
the determining equations for the symmetry group of the given
system. In this case, we find the determining equations for the
symmetry group of the system (\ref{eq:1}) to be the following:
%
\be \label{eq:3}
%
&&\hspace{-1cm} \xi_{1,t^2}=\xi_{1,x}=\xi_{1,y}=\xi_{1,z}=\xi_{1,u}=\xi_{1,v}=\xi_{1,w}=\xi_{1,q}=\xi_{1,p}=0,\nonumber\\
%
&&\hspace{-1cm} \xi_{2,x}=\xi_{2,u}=\xi_{2,v}=\xi_{2,w}=\xi_{2,q}=\xi_{2,p}=\xi_{2,t^2}=\xi_{2,ty}=\xi_{2,y^2}=0,\nonumber\\
%
&&\hspace{-1cm} \xi_{3,y}=\xi_{3,u}=\xi_{3,v}=\xi_{3,w}=\xi_{3,q}=\xi_{3,p}=\xi_{3,t^2}=\xi_{4,z}=\xi_{4,w}=\xi_{4,q}=0,\\
%
&&\hspace{-1cm} \xi_{4,p}=\xi_{4,t^2}=\xi_{4,tx}=\xi_{4,ty}=\xi_{4,x^2}=\xi_{4,xy}=\xi_{4,y^2}=0,\nonumber\\
%
&&\hspace{-1cm}
\xi_{3,x}=\xi_{2,y},\,\xi_{3,z}+\xi_{4,y}=0,\,\xi_{4,v}=\xi_{4,u},\,\xi_{2,z}+\xi_{4,x}=0,\nonumber\\[2mm]
%
&&\hspace{-1cm}
\eta_1=-u\xi_{1,t}+\xi_{2,t}+v\xi_{2,y}-w\xi_{4,x},\quad\eta_2=-w\xi_{4,y}+\xi_{3,t}-u\xi_{2,y}-v\xi_{1,t},\nonumber\\
%
&&\hspace{-1cm}
\eta_3=u\xi_{4,x}+\xi_{4,t}+v\xi_{4,y}-w\xi_{1,t},\label{eq:4}\quad \eta_4=q\eta_{5}/p+2q\xi_{1,t},\\
%
&&\hspace{-1cm}
\eta_{5,t}=\eta_{5,x}=\eta_{5,y}=\eta_{5,z}=\eta_{5,u}=\eta_{5,v}=\eta_{5,w}=\eta_{5,q}=0,\quad
\eta_{5}=p\eta_{5,p}.\nonumber \ee
%
First, equations (\ref{eq:3}) require that $\xi_i$s are just
%
\begin{align}\label{eq:5}
%
& \xi_1=a_1t+a_2, && \xi_2=a_3t+a_4x+a_5y+a_6z+a_7,\nonumber
\\[-3mm]\\[-2mm]
& \xi_3=a_8t-a_5x+a_4y+a_9z+a_{10},&&
\xi_4=a_{11}t-a_6x-a_9y+a_4z+a_{12},\nonumber
%
\end{align}
%
where $a_1,\cdots,a_{12}$ are arbitrary constants. Then, equations
(\ref{eq:4}) and (\ref{eq:5}) requires that
%
\be \label{eq:6} &&\hspace{-3mm}
\eta_1=(a_4-a_1)u+a_5v-a_6w+a_3,\qquad
\eta_2=-a_5u+(a_4-a_1)v+a_4w+a_8,\nonumber
\\[-3mm] \\[-2mm]
&&\hspace{-3mm} \eta_3=-a_6u-a_9v+(a_4-a_1)w+a_{11},\quad
\eta_4=(2a_1-2a_4+a_{13})q,\quad \eta_5=a_{13}p,\nonumber \ee
%
where $a_{13}$ is an arbitrary constant. Therefore
%
\paragraph{Theorem 1.}
%
{\em The Lie algebra of infinitesimal symmetries of the system
(\ref{eq:1}) is spanned by the 13 vector fields
%
\be
%
\begin{array}{lll}
X_1 = \partial_x,\qquad X_2 = \partial_y,&&\hspace{-3cm}\mbox{(shifts of origin)}\\
X_3 = \partial_z,\qquad X_4 = \partial_t,&&\\ \\
X_5 = t\,\partial_x+\partial_u,&&\\
X_6 = t\,\partial_y+\partial_v,&&\hspace{-3cm}\mbox{(uniformly frame motions)}\\
X_7 = t\,\partial_z+\partial_w,&&\\ \\
X_8 = t\,\partial_t-u\,\partial_u-v\,\partial_v-w\,\partial_w+2q\,\partial_q,\\
X_9 =
x\,\partial_x+y\,\partial_y+z\,\partial_z+u\,\partial_u+v\,\partial_v+w\,\partial_w-2r\,\partial_r,\label{eq:7}\\
\\
X_{10} = y\,\partial_x-x\,\partial_y+v\,\partial_u-u\,\partial_v,&&\\
X_{11} = -z\,\partial_y+y\,\partial_z-w\,\partial_v+v\,\partial_w,&&\hspace{-3cm}\mbox{(rotations of reference frame)}\\
X_{12} =
-z\,\partial_x+x\,\partial_z-w\,\partial_u+u\,\partial_w,&&\\ \\
X_{13} = q\,\partial_q+p\,\partial_p,
\end{array}
%
\ee
%
These infinitesimal symmetries will generate a Lie algebra $\bf g$
over the field of real or complex numbers. The commutator table of
Lie algebra $\bf g$ for (\ref{eq:1}) is given in Table 1, where
the entry in the $i$th row and $j$th column is defined as
$[X_i,X_j]=X_i.X_j-X_j.X_i$, $i,j=1,\cdots,13$.}
%
%
\section{Reduction of the system}
%
Now, we look at the group-invariant solutions to the system
(\ref{eq:1}).

\medskip The system (\ref{eq:1}) is a sub-manifold $M$ of jet space
$J^2(\RR^4,\RR^5)$ defined by the following equations
%
\be
%
&&\hspace{-1cm} u_t+uu_x+vu_y+wu_z +p_x/q=0,\nonumber \\
%
&&\hspace{-1cm} v_t+uv_x+vv_y+wv_z+p_y/q=0,\nonumber \\
%
&&\hspace{-1cm} w_t+uw_x+vw_y+ww_z+p_z/q=0,\label{eq:2}\\
%
&&\hspace{-1cm} q_t+q \left(u_x+v_y+w_z\right)+uq_x+vq_y+wq_z=0,\nonumber \\
%
&&\hspace{-1cm}
p_t+\gamma\,p\left(u_x+v_y+w_z\right)+up_x+vp_y+wp_z=0.\nonumber
%
\ee
%
%
\begin{eqnarray*}
%
&&\hspace{4cm} \mbox{Table 1}\\ && \hspace{-0.7cm}\small
\begin{array}{|c|ccccccccccccc|}
\hline\   \!\!&\!\!X_1\!\!&\!\!X_2\!\!&\!\!X_3\!\!&\!\!X_4\!\!&\!\!X_5\!\!&\!\!X_6\!\!&\!\!X_7\!\!&\!\!X_8\!\!&\!\!X_9\!\!&\!\!X_{10}\!\!&\!\!X_{11}\!\!&\!\!X_{12}\!\!&\!\!X_{13}\\
\hline\ X_1\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!X_1\!\!&\!\!-X_2\!\!&\!\!0\!\!&\!\!X_3\!\!&\!\!0\\
X_2\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!X_2\!\!&\!\!X_1\!\!&\!\!X_3\!\!&\!\!0\!\!&\!\!0\\
X_3\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!X_3\!\!&\!\!0\!\!&\!\!-X_2\!\!&\!\!-X_1\!\!&\!\!0\\
X_4\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!X_1\!\!&\!\!X_2\!\!&\!\!X_3\!\!&\!\!X_4\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\\
X_5\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_1\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_5\!\!&\!\!X_5\!\!&\!\!-X_6\!\!&\!\!0\!\!&\!\!X_7\!\!&\!\!0\\
X_6\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_2\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_6\!\!&\!\!X_6\!\!&\!\!X_5\!\!&\!\!X_7\!\!&\!\!0\!\!&\!\!0\\
X_7\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_3\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_7\!\!&\!\!X_7\!\!&\!\!0\!\!&\!\!-X_6\!\!&\!\!-X_5\!\!&\!\!0\\
X_8\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_4\!\!&\!\!X_5\!\!&\!\!X_6\!\!&\!\!X_7\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\\
X_9\!\!&\!\!-X_1\!\!&\!\!-X_2\!\!&\!\!-X_3\!\!&\!\!0\!\!&\!\!-X_5\!\!&\!\!-X_6\!\!&\!\!-X_7\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\\
X_{10}\!\!&\!\!X_2\!\!&\!\!-X_1\!\!&\!\!0\!\!&\!\!0\!\!&\!\!X_6\!\!&\!\!-X_5\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_{12}\!\!&\!\!X_{11}\!\!&\!\!0\\
X_{11}\!\!&\!\!0\!\!&\!\!-X_3\!\!&\!\!X_2\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_7\!\!&\!\!X_6\!\!&\!\!0\!\!&\!\!0\!\!&\!\!X_{12}\!\!&\!\!0\!\!&\!\!-X_{10}\!\!&\!\!0\\
X_{12}\!\!&\!\!-X_3\!\!&\!\!0\!\!&\!\!X_1\!\!&\!\!0\!\!&\!\!-X_7\!\!&\!\!0\!\!&\!\!X_5\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-X_{11}\!\!&\!\!X_{10}\!\!&\!\!0\!\!&\!\!0\\
X_{13}\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\\
\hline
\end{array}
%
\end{eqnarray*}

Doing as section 3.1 of \cite{Olv2} (or \cite{NadHej,Udr}) and
find (in a sense) the most general group-invariant solutions to
the system (\ref{eq:1}).
%
\paragraph{Theorem 2.}
%
{\em The one-parameter groups $g_i(s):M\to M$ generated by the
$X_i$, $i=1,\cdots,13$ are given in the following table:
%
\begin{align}
g_1 &: \big(t,x+s,y,z,u,v,w,p,q\big),\qquad g_2 : \big(t,x,y+s,z,u,v,w,p,q\big),\nonumber\\
g_3 &: \big(t,x,y,z+s,u,v,w,p,q\big),\qquad g_4 : \big(t+s,x,y,z,u,v,w,p,q\big),\nonumber\\
g_5 &: \big(t,x+st,y,z,u+s,v,w,p,q\big), \nonumber\\
g_6 &: \big(t,x,y+st,z,u,v+s,w,p,q\big), \nonumber \\
g_7 &: \big(t,x,y,z+st,u,v,w+s,p,q\big), \label{eq:8}\\
g_8 &: \big(e^st,x,y,z,e^{-s}u,e^{-s}v,e^{-s}w,p,e^{2s}q\big),
\nonumber\\
g_9 &: \big(t,e^sx,e^sy,e^sz,e^su,e^sv,e^sw,p,e^{-2s}q\big), \nonumber\\
g_{10} &: \big(t,x\cos s+y\sin s,y\cos s-x\sin s,z,\nonumber\\
& \hspace{3cm} v\sin s+u\cos s,v\cos s-u\sin s,w,p,q\big),
\nonumber\end{align}
\begin{align}
g_{11} &: \big(t,x,y\cos s-z\sin s,z\cos s+y\sin s,\nonumber\\
& \hspace{3cm} u,v\cos s-w\sin s,w\cos s+v\sin s,p,q\big), \nonumber\\
g_{12} &: \big(t,x\cos s-z\sin s,y,x\sin s+z\cos s,\nonumber\\
& \hspace{3cm} u\cos s-w\sin s,v,w\cos s+u\sin s,p,q\big), \nonumber\\
g_{13} &: \big(t,x,y,z,u,v,w,e^sp,e^sq\big). \nonumber
%
\end{align}
%
Where, entries give the transformed point
$$\exp(sX_i)(t,x,y,z,u,v,w,p,q) =
(\tilde{t},\tilde{x},\tilde{y},\tilde{z},\tilde{u},\tilde{v},\tilde{w},\tilde{p},\tilde{q}).$$}

\medskip Since each group $g_i$, $i=1,\cdots,13$, is a symmetry
group of (\ref{eq:1}), then
%
\paragraph{Theorem 3.}
%
{\em Let $i=1,\cdots,13$, $s\in\RR$, and $\lambda\in\RR-\{0\}$. If
%
\begin{eqnarray*}
&& u=U(t,x,y,z),\;v=V(t,x,y,z),\;w=W(t,x,y,z),\\
&& p=P(t,x,y,z),\;q=Q(t,x,y,z),
\end{eqnarray*}
%
is a solution of the system (\ref{eq:1}), so are the functions
%
\begin{eqnarray*}
&& u^{(i)}=U^{(i)}(t,x,y,z),\;v^{(i)}=V^{(i)}(t,x,y,z),\;w^{(i)}=W^{(i)}(t,x,y,z),\\
&& p^{(i)}=P^{(i)}(t,x,y,z),\;q^{(i)}=Q^{(i)}(t,x,y,z),
\end{eqnarray*}
%
where
%
\be
\begin{array}{llll}
u^{(1)}\,=\,U\big(t,x+s,y,z\big), &&& u^{(2)}\,=\,U\big(t,x,y+s,z\big),\\
v^{(1)}\,=\,V\big(t,x+s,y,z\big), &&& v^{(2)}\,=\,V\big(t,x,y+s,z\big),\\
w^{(1)}\,=\,W\big(t,x+s,y,z\big), &&& w^{(2)}\,=\,W\big(t,x,y+s,z\big),\\
p^{(1)}\,=\,P\big(t,x+s,y,z\big), &&& p^{(2)}\,=\,P\big(t,x,y+s,z\big),\\
q^{(1)}\,=\,Q\big(t,x+s,y,z\big). &&&
q^{(2)}\,=\,Q\big(t,x,y+s,z\big).
\end{array} \nonumber
\ee
%
%
\be
\begin{array}{llll}
u^{(3)}\,=\,U\big(t,x,y,z+s\big), &&& u^{(4)}\,=\,U\big(t+s,x,y,z\big),\\
v^{(3)}\,=\,V\big(t,x,y,z+s\big), &&& v^{(4)}\,=\,V\big(t+s,x,y,z\big),\\
w^{(3)}\,=\,W\big(t,x,y,z+s\big), &&& w^{(4)}\,=\,W\big(t+s,x,y,z\big),\\
p^{(3)}\,=\,P\big(t,x,y,z+s\big), &&& p^{(4)}\,=\,P\big(t+s,x,y,z\big),\\
q^{(3)}\,=\,Q\big(t,x,y,z+s\big). &&&
q^{(4)}\,=\,Q\big(t+s,x,y,z\big).
\end{array} \nonumber
\ee
%
%
\be
\begin{array}{llll}
u^{(5)}\,=\,U\big(t,x+st,y,z\big)-s, &&& u^{(6)}\,=\,U\big(t,x,y+st,z\big),\\
v^{(5)}\,=\,V\big(t,x+st,y,z\big),   &&& v^{(6)}\,=\,V\big(t,x,y+st,z\big)-s,\\
w^{(5)}\,=\,W\big(t,x+st,y,z\big),   &&& w^{(6)}\,=\,W\big(t,x,y+st,z\big),\\
p^{(5)}\,=\,P\big(t,x+st,y,z\big),   &&& p^{(6)}\,=\,P\big(t,x,y+st,z\big),\\
q^{(5)}\,=\,Q\big(t,x+st,y,z\big).   &&&
q^{(6)}\,=\,Q\big(t,x,y+st,z\big).
\end{array} \nonumber
\ee
%
%
\be
\begin{array}{llll}
u^{(7)}\,=\,U\big(t,x,y,z+st\big),   &&& u^{(8)}\,=\,\lambda.U\big(\lambda.t,x,y,z\big),\\
v^{(7)}\,=\,V\big(t,x,y,z+st\big),   &&& v^{(8)}\,=\,\lambda.V\big(\lambda.t,x,y,z\big),\\
w^{(7)}\,=\,W\big(t,x,y,z+st\big)-s, &&& w^{(8)}\,=\,\lambda.W\big(\lambda.t,x,y,z\big),\\
p^{(7)}\,=\,P\big(t,x,y,z+st\big),   &&& p^{(8)}\,=\,P\big(\lambda.t,x,y,z\big),\\
q^{(7)}\,=\,Q\big(t,x,y,z+st\big).   &&&
q^{(8)}\,=\,\frac{1}{\lambda^2}.Q\big(\lambda.t,x,y,z\big).
\end{array} \nonumber
\ee
%
%
\be
\begin{array}{llll}
u^{(9)}\,=\,\frac{1}{\lambda}.U\big(t,\lambda.x,\lambda.y,\lambda.z\big), &&& u^{(13)}\,=\,U\big(t,x,y,z\big),\\
v^{(9)}\,=\,\frac{1}{\lambda}.V\big(t,\lambda.x,\lambda.y,\lambda.z\big), &&& v^{(13)}\,=\,V\big(t,x,y,z\big),\\
w^{(9)}\,=\,\frac{1}{\lambda}.W\big(t,\lambda.x,\lambda.y,\lambda.z\big), &&& w^{(13)}\,=\,W\big(t,x,y,z\big),\\
p^{(9)}\,=\,P\big(t,\lambda.x,\lambda.y,\lambda.z\big),                   &&& p^{(13)}\,=\,\lambda.P\big(t,x,y,z\big),\\
q^{(9)}\,=\,\lambda^2.Q\big(t,\lambda.x,\lambda.y,\lambda.z\big).
&&& q^{(13)}\,=\,\lambda.Q\big(t,x,y,z\big).
\end{array} \nonumber
\ee
%
%
\be
u^{(10)}&=&\cos s.U\big(t,x\cos s+y\sin s,y\cos s-x\sin s,z\big)\nonumber\\
&& -\sin s.V\big(t,x\cos s+y\sin s,y\cos s-x\sin s,z\big),\nonumber\\
v^{(10)}&=&\sin s.U\big(t,x\cos s+y\sin s,y\cos s-x\sin s,z\big)\nonumber\\
&&+\cos s.V\big(t,x\cos s+y\sin s,y\cos s-x\sin s,z\big),\nonumber\\
w^{(10)}&=&W\big(t,x\cos s+y\sin s,y\cos s-x\sin s,z\big),\nonumber\\
p^{(10)}&=&P\big(t,x\cos s+y\sin s,y\cos s-x\sin s,z\big),\nonumber\\
q^{(10)}&=&Q\big(t,x\cos s+y\sin s,y\cos s-x\sin
s,z\big).\nonumber \ee
%
%
\be
u^{(11)}&=&U\big(t,x,y\cos s-z\sin s,z\cos s+y\sin s\big),\nonumber\\
v^{(11)}&=&\cos s.V\big(t,x,y\cos s-z\sin s,z\cos s+y\sin s\big)\nonumber\\
&&+\sin s.W\big(t,x,y\cos s-z\sin s,z\cos s+y\sin s\big),\nonumber\\
w^{(11)}&=&\cos s.W\big(t,x,y\cos s-z\sin s,z\cos s+y\sin s\big)\nonumber\\
&&-\sin s.V\big(t,x,y\cos s-z\sin s,z\cos s+y\sin
s\big),\nonumber\\
p^{(11)}&=&P\big(t,x,y\cos s-z\sin s,z\cos s+y\sin s\big),\nonumber\\
q^{(11)}&=&Q\big(t,x,y\cos s-z\sin s,z\cos s+y\sin
s\big).\nonumber \ee
%
%
\be
u^{(12)}&=&\cos s.U\big(t,x\cos s-z\sin s,y,x\sin s+z\cos s\big)\nonumber\\
&&+\sin s.W\big(t,x\cos s-z\sin s,y,x\sin s+z\cos s\big),\nonumber\\
v^{(12)}&=&V\big(t,x\cos s-z\sin s,y,x\sin s+z\cos s\big),\nonumber\\
w^{(12)}&=&\cos s.W\big(t,x\cos s-z\sin s,y,x\sin s+z\cos s\big)\nonumber\\
&&-\sin s.U\big(t,x\cos s-z\sin s,y,x\sin s+z\cos
s\big),\nonumber\\
p^{(12)}&=&P\big(t,x\cos s-z\sin s,y,x\sin s+z\cos s\big),\nonumber\\
q^{(12)}&=&Q\big(t,x\cos s-z\sin s,y,x\sin s+z\cos
s\big)\nonumber. \ee}
%
%
\section{Structure of Lie algebra $\bf g$}
%
%
In this section, we determine the structure of full symmetry
algebra $\bf g$. of system (\ref{eq:1}).

The center $\bf z$ of $\bf g$ is $\Span_\RR\{X_{13}\}$. Therefore,
the quotient algebra ${\bf g}_1:={\bf g}/{\bf z}$ is
$\Span_\RR\{Y_1,\cdots,Y_{12}\}$; where $Y_i:=X_i+{\bf z}$,
$i=1,\cdots,12$. The commutator table of Lie algebra ${\bf g}_1$
is given in Table 2, where the entry in the $i$th row and $j$th
column is defined as $[Y_i,Y_j]=Y_i.Y_j-Y_j.Y_i$,
$i,j=1,\cdots,12$.
%
\begin{eqnarray*}
%
&&\hspace{4cm}\mbox{Table 2}\\&& \hspace{-1.3cm}\small
\begin{array}{|c|cccccccccccc|}
\hline\   \!\!&\!\!Y_1\!\!&\!\!Y_2\!\!&\!\!Y_3\!\!&\!\!Y_4\!\!&\!\!Y_5\!\!&\!\!Y_6\!\!&\!\!Y_7\!\!&\!\!Y_8\!\!&\!\!Y_9\!\!&\!\!Y_{10}\!\!&\!\!Y_{11}\!\!&\!\!Y_{12}\\
\hline\ Y_1\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!Y_1\!\!&\!\!-Y_2\!\!&\!\!0\!\!&\!\!Y_3\\
Y_2\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!Y_2\!\!&\!\!Y_1\!\!&\!\!Y_3\!\!&\!\!0\\
Y_3\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!Y_3\!\!&\!\!0\!\!&\!\!-Y_2\!\!&\!\!-Y_1\\
Y_4\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!Y_1\!\!&\!\!Y_2\!\!&\!\!Y_3\!\!&\!\!Y_4\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\\
Y_5\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_1\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_5\!\!&\!\!Y_5\!\!&\!\!-Y_6\!\!&\!\!0\!\!&\!\!Y_7\\
Y_6\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_2\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_6\!\!&\!\!Y_6\!\!&\!\!Y_5\!\!&\!\!Y_7\!\!&\!\!0\\
Y_7\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_3\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_7\!\!&\!\!Y_7\!\!&\!\!0\!\!&\!\!-Y_6\!\!&\!\!-Y_5\\
Y_8\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_4\!\!&\!\!Y_5\!\!&\!\!Y_6\!\!&\!\!Y_7\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\\
Y_9\!\!&\!\!-Y_1\!\!&\!\!-Y_2\!\!&\!\!-Y_3\!\!&\!\!0\!\!&\!\!-Y_5\!\!&\!\!-Y_6\!\!&\!\!-Y_7\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\\
Y_{10}\!\!&\!\!Y_2\!\!&\!\!-Y_1\!\!&\!\!0\!\!&\!\!0\!\!&\!\!Y_6\!\!&\!\!-Y_5\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_{12}\!\!&\!\!Y_{11}\\
Y_{11}\!\!&\!\!0\!\!&\!\!-Y_3\!\!&\!\!Y_2\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_7\!\!&\!\!Y_6\!\!&\!\!0\!\!&\!\!0\!\!&\!\!Y_{12}\!\!&\!\!0\!\!&\!\!-Y_{10}\\
Y_{12}\!\!&\!\!-Y_3\!\!&\!\!0\!\!&\!\!Y_1\!\!&\!\!0\!\!&\!\!-Y_7\!\!&\!\!0\!\!&\!\!Y_5\!\!&\!\!0\!\!&\!\!0\!\!&\!\!-Y_{11}\!\!&\!\!Y_{10}\!\!&\!\!0\\
\hline
\end{array}
%
\end{eqnarray*}
%
The algebra ${\bf g}_1$ is not solvable, because ${\bf
g}_1^{(1)}:=[{\bf g}_1,{\bf g}_1]=\Span_\RR\{Y_1,\cdots,Y_{10}\}$
and ${\bf g}_1^{(2)}:=[{\bf g}_1^{(1)},{\bf g}_1^{(1)}]={\bf
g}_1^{(1)}$. Lie algebra ${\bf g}_1$ admits a Levi-decomposition
into the semi-direct sum ${\bf g}_1={\bf r}\ltimes{\bf s}$, where
${\bf r}=\Span_\RR\{Y_1,\cdots,Y_9\}$ is the radical of ${\bf
g}_1$ (the largest solvable ideal contained in ${\bf g}_1$) and
${\bf s}=\Span_\RR\{Y_{10},Y_{11},Y_{12}\}$ is a semi-simple
subalgebra of ${\bf g}_1$. The radical $\bf r$ is uniquely defined
but the semi-simple subalgebra $\bf s$ is not. $\bf s$ as an
algebra is isomorphic to $3-$dimensional special orthogonal
algebra ${\bf so}(3):=\{A\in\mathrm{Mat}(3\times
3;\RR)\,|\,A^t=-A\}$, which is a simple algebra. The radical ${\bf
r}$ is solvable, with and ${\bf
r}^{(1)}=\Span_\RR\{Y_1,\cdots,Y_7\}$, ${\bf
r}^{(2)}=\Span_\RR\{Y_1,Y_2,Y_3\}$, ${\bf r}^{(3)}=\{0\}$. It is
semi-direct sum ${\bf r}={\bf r}^{(1)}\ltimes {\bf g}_2$, where
${\bf g}_2=\Span_\RR\{Y_8,Y_9\}$ is isomorphic to the two
dimensional Abelian Lie algebra $\RR^2$; i.e. ${\bf r}={\bf
r}^{(1)}\ltimes \RR^2$.

${\bf r}^{(1)}$ is semi-direct sum ${\bf r}^{(1)}={\bf
r}^{(2)}\ltimes {\bf g}_3,$ where ${\bf
g}_3=\Span_\RR\{Y_4,\cdots,Y_7\}$ is isomorphic to the four
dimensional Abelian Lie algebra $\RR^4$, and ${\bf r}^{(2)}$ is
isomorphic to the three dimensional Abelian Lie algebra $\RR^3$;
i.e. ${\bf r}^{(1)}=\RR^3\ltimes \RR^4.$
%
\paragraph{Theorem 4.}
{\em The symmetry algebra $\bf g$ of system (\ref{eq:1}) have the
following structure ${\bf
g}\cong\RR\times(((\RR^3\ltimes\RR^4)\ltimes\RR^2)\ltimes{\bf
so}(3)).$}
%
\paragraph{Theorem 5.} (see
\cite{NadMeh}) {\em There is a normal Lie-subalgebra of symmetry
Lie-group of system (\ref{eq:1}) which is isomorphic to the
Galilean group of
$\RR^4$: $${\rm Gal}(4,{\Bbb R})=\left\{ \left(\begin{array}{ccc} 1 & {\bf 0} & s \\ {\bf v} & {\bf R} & {\bf y} \\
0 & {\bf 0} & 1
\end{array}\right)\;\Big|\; {\bf R}\in{\rm
O}(3,{\Bbb R}),\; s\in{\Bbb R},\; \mbox{and}\;\; {\bf y},{\bf
v}\in{\Bbb R}^3 \;\right\}.$$ Therefore, the system (\ref{eq:1})
is invariant up to Galilean motions of space-times $\RR^4$ .}
%

\medskip \noindent {\it Proof.} Let
${\bf b}=\Span_\RR\{X_1,\cdots,X_7,X_{10},X_{11},X_{12}\}$. Lie
algebra structure of ${\bf b}$ is as ${\bf gal}(3)$, the lie
algebra of Galilean group ${\rm Gal}(4,{\Bbb R})$, and $\bf b$ an
ideal of $\bf g$. Therefore, there is a Lie-subgroup of $G$ such
that its Lie-algebra is $\bf b$, by the Theorem 2.53 of Olver
\cite{Olv2}. \hfill\ $\Box$
%
\paragraph{Conclusion 1.}
%
{\em $\bf g$ is semi-direct sum of ${\bf
gal}(4)\cong\Span_\RR\{X_1,\cdots,X_7,X_{10},X_{11},X_{12}\}$ and
$3-$dimensional Abelian algebra
$\RR^3\cong\Span\{X_8,X_9,X_{13}\}$.}
%
%
\section{Optimal system of sub-algebras}
%
%
As is well known, the Lie group theoretic method plays an
important role in finding exact solutions and performing symmetry
reductions of differential equations. Since any linear combination
of infinitesimal generators is also an infinitesimal generator,
there are always infinitely many different symmetry subgroups for
the differential equation. So, a mean of determining which
subgroups would give essentially different types of solutions is
necessary and significant for a complete understanding of the
invariant solutions. As any transformation in the full symmetry
group maps a solution to another solution, it is sufficient to
find invariant solutions which are not related by transformations
in the full symmetry group, this has led to the concept of an
optimal system \cite{Ovs}. The problem of finding an optimal
system of subgroups is equivalent to that of finding an optimal
system of subalgebras. For one-dimensional subalgebras, this
classification problem is essentially the same as the problem of
classifying the orbits of the adjoint representation. This problem
is attacked by the naive approach of taking a general element in
the Lie algebra and subjecting it to various adjoint
transformations so as to simplify it as much as possible. The idea
of using the adjoint representation to classify group-invariant
solutions was due to \cite{Ovs} and \cite{NadHej,Udr}.

The adjoint action is given by the Lie series
%
\be \mathrm{Ad}(\exp(sX_i)X_j) =
X_j-s[X_i,X_j]+\frac{s^2}{2}[X_i,[X_i,X_j]]-\cdots,\ee
%
where $[X_i,X_j]$ is the commutator for the Lie algebra, $s$ is a
parameter, and $i,j=1,\cdots,13$. We can write the adjoint action
for the Lie algebra $\bf g$, and show that
%
\paragraph{Theorem 6.}
{\em A one-dimensional optimal system of (\ref{eq:1}) is given by
\begin{align*}
1)&\;\;X_8+\sum_{i=9}^{13}a_iX_i, &
2)&\;\;a_7X_7+X_8+X_9+\sum_{i=10}^{13}a_iX_i,\\
3)&\;\;a_6X_6+a_7X_7+X_8+X_9+\sum_{i=11}^{13}a_iX_i, &
4)&\;\;a_5X_5+X_8+X_9+a_{11}X_i+a_{13}X_{13}, \\
5)&\;\;\sum_{i=5}^7a_iX_i+X_8+X_9+a_{13}X_{13},&
6)&\;\;a_4X_4+X_9+\sum_{i=10}^{13}a_iX_i,\\
7)&\;\;X_4+a_5X_5+a_8X_8+\sum_{i=10}^{13}a_iX_i,&
8)&\;\;X_4+a_6X_6+a_8X_8+\sum_{i=10}^{13}a_iX_i,\end{align*}
\begin{align*}
9)&\;\;X_4+a_7X_7+a_8X_8+\sum_{i=10}^{13}a_iX_i,&
10)&\;\;X_4+\sum_{i=5}^8a_iX_i+a_{13}X_{13},\\
11)&\;\;X_4+a_7X_7+\sum_{i=10}^{13}a_iX_i,&
12)&\;\;X_7+\sum_{i=10}^{13}a_iX_i,\\
13)&\;\;a_3X_3+\sum_{i=10}^{13}a_iX_i,&
14)&\;\;X_4+a_6X_6+\sum_{i=11}^{13}a_iX_i,\\
15)&\;\;X_4+a_5X_5+a_{11}X_{11}+a_{13}X_{13},&
16)&\;\;X_4+\sum_{i=5}^7a_iX_i+a_{13}X_{13},\\
17)&\;\;X_6+\sum_{i=11}^{13}a_iX_i,&
18)&\;\;a_2X_2+\sum_{i=11}^{13}a_iX_i,\\
19)&\;\;a_2X_2+a_{12}X_{12}+a_{13}X_{13},&
20)&\;\;X_5+a_{11}X_{11}+a_{13}X_{13},\\
21)&\;\;a_2X_2+a_3X_3+X_5+a_{13}X_{13},&
22)&\;\;a_1X_1+X_{11}+a_{13}X_{13},\\
23)&\;\;a_1X_1+a_3X_3+X_6+a_{13}X_{13},&
24)&\;\;a_1X_1+a_2X_2+a_3X_3+a_{13}X_{13},\\
25)&\;\;X_5+a_{10}X_{10}+a_{11}X_{11}+a_{13}X_{13},&
26)&\;\;a_3X_3+X_{10}+a_{11}X_{11}+a_{13}X_{13}.
\end{align*}}
%
\medskip \noindent {\it Proof:} $F(sX_i):{\bf g}\to{\bf g}$ defined by
$X\mapsto\mathrm{Ad}(\exp(sX_i)X)$ is a linear map, for
$i=1,\cdots,13$. The matrix $M_{sX_i}$ of $F(sX_i)$,
$i=1,\cdots,13$, with respect to basis $\{X_1,\cdots,X_{13}\}$ is
%
\be
%
&&\hspace{-1cm} \tiny \left[\begin{array}{ccccccccccccc}
1&0&0&0&0&0&0&0&0&0&0&0&0\\0&1&0&0&0&0&0&0&0&0&0&0&0\\0&0&1
&0&0&0&0&0&0&0&0&0&0\\0&0&0&1&0&0&0&0&0&0&0&0&0
\\0&0&0&0&1&0&0&0&0&0&0&0&0\\0&0&0
&0&0&1&0&0&0&0&0&0&0\\0&0&0&0&0&0&1&0&0&0&0&0&0
\\0&0&0&0&0&0&0&1&0&0&0&0&0\\-s&0&0
&0&0&0&0&0&1&0&0&0&0\\0&s&0&0&0&0&0&0&0&1&0&0&0
\\0&0&0&0&0&0&0&0&0&0&1&0&0\\0&0&-
s&0&0&0&0&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
\end{array}\right],\cdots\nonumber \\[-3mm] \\[-2mm]
%
%&&\hspace{-1cm} \tiny \left[\begin{array}{ccccccccccccc}
%1&0&0&0&0&0&0&0&0&0&0&0&0
%\\0&1&0&0&0&0&0&0&0&0&0&0&0\\0&0&1
%&0&0&0&0&0&0&0&0&0&0\\0&0&0&1&0&0&0&0&0&0&0&0&0
%\\0&0&0&0&1&0&0&0&0&0&0&0&0\\0&0&0
%&0&0&1&0&0&0&0&0&0&0\\0&0&0&0&0&0&1&0&0&0&0&0&0
%\\0&0&0&0&0&0&0&1&0&0&0&0&0\\0&-s&0
%&0&0&0&0&0&1&0&0&0&0\\-s&0&0&0&0&0&0&0&0&1&0&0&0
%\\0&0&-s&0&0&0&0&0&0&0&1&0&0\\0&0&0
%&0&0&0&0&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
%\end{array}\right],\nonumber \\[3mm]
%
%&&\hspace{-1cm} \tiny \left[\begin{array}{ccccccccccccc}
%1&0&0&0&0&0&0&0&0&0&0&0&0\\0&1&0&0&0&0&0&0&0&0&0&0&0\\0&0&1
%&0&0&0&0&0&0&0&0&0&0\\0&0&0&1&0&0&0&0&0&0&0&0&0
%\\0&0&0&0&1&0&0&0&0&0&0&0&0\\0&0&0
%&0&0&1&0&0&0&0&0&0&0\\0&0&0&0&0&0&1&0&0&0&0&0&0
%\\0&0&0&0&0&0&0&1&0&0&0&0&0\\0&0&-
%s&0&0&0&0&0&1&0&0&0&0\\0&0&0&0&0&0&0&0&0&1&0&0&0
%\\0&s&0&0&0&0&0&0&0&0&1&0&0\\s&0&0
%&0&0&0&0&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
%\end{array}\right],
%\nonumber \\[3mm]
%%
%&&\hspace{-1cm} \tiny \left[\begin{array}{ccccccccccccc}
%1&0&0&0&0&0&0&0&0&0&0&0&0\\0&1&0&0&0&0&0&0&0&0&0&0&0\\0&0&1
%&0&0&0&0&0&0&0&0&0&0\\0&0&0&1&0&0&0&0&0&0&0&0&0
%\\-s&0&0&0&1&0&0&0&0&0&0&0&0\\0&-s
%&0&0&0&1&0&0&0&0&0&0&0\\0&0&-s&0&0&0&1&0&0&0&0&0&0
%\\0&0&0&-s&0&0&0&1&0&0&0&0&0\\0&0&0
%&0&0&0&0&0&1&0&0&0&0\\0&0&0&0&0&0&0&0&0&1&0&0&0
%\\0&0&0&0&0&0&0&0&0&0&1&0&0\\0&0&0
%&0&0&0&0&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
%\end{array}\right],\nonumber \\[3mm]
%%
%&&\hspace{-1cm} \tiny \left[\begin{array}{ccccccccccccc}
%1&0&0&0&0&0&0&0&0&0&0&0&0
%\\0&1&0&0&0&0&0&0&0&0&0&0&0\\0&0&1
%&0&0&0&0&0&0&0&0&0&0\\s&0&0&1&0&0&0&0&0&0&0&0&0
%\\0&0&0&0&1&0&0&0&0&0&0&0&0\\0&0&0
%&0&0&1&0&0&0&0&0&0&0\\0&0&0&0&0&0&1&0&0&0&0&0&0
%\\0&0&0&0&s&0&0&1&0&0&0&0&0\\0&0&0
%%\\0&0&0&0&0&0&0&0&0&0&1&0&0\\0&0&0
%&0&0&0&-s&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
%\end{array}\right],\nonumber \\[3mm]
%
%&&\hspace{-1cm} \tiny \left[\begin{array}{ccccccccccccc}
%1&0&0&0&0&0&0&0&0&0&0&0&0
%\\0&1&0&0&0&0&0&0&0&0&0&0&0\\0&0&1
%&0&0&0&0&0&0&0&0&0&0\\0&s&0&1&0&0&0&0&0&0&0&0&0
%\\0&0&0&0&1&0&0&0&0&0&0&0&0\\0&0&0
%&0&0&1&0&0&0&0&0&0&0\\0&0&0&0&0&0&1&0&0&0&0&0&0
%\\0&0&0&0&0&s&0&1&0&0&0&0&0\\0&0&0
%&0&0&-s&0&0&1&0&0&0&0\\0&0&0&0&-s&0&0&0&0&1&0&0&0
%\\0&0&0&0&0&0&-s&0&0&0&1&0&0\\0&0&0
%&0&0&0&0&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
%\end{array}\right],
%\nonumber \\[3mm]
%
%&&\hspace{-1cm} \tiny \left[\begin{array}{ccccccccccccc}
%1&0&0&0&0&0&0&0&0&0&0&0&0\\0&1&0&0&0&0&0&0&0&0&0&0&0\\0&0&1
%&0&0&0&0&0&0&0&0&0&0\\0&0&s&1&0&0&0&0&0&0&0&0&0
%\\0&0&0&0&1&0&0&0&0&0&0&0&0\\0&0&0
%&0&0&1&0&0&0&0&0&0&0\\0&0&0&0&0&0&1&0&0&0&0&0&0
%\\0&0&0&0&0&0&s&1&0&0&0&0&0\\0&0&0
%&0&0&0&-s&0&1&0&0&0&0\\0&0&0&0&0&0&0&0&0&1&0&0&0
%\\0&0&0&0&0&s&0&0&0&0&1&0&0\\0&0&0
%&0&s&0&0&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
%\end{array}\right],\nonumber \\[3mm]
%
%&&\hspace{-1cm} \tiny \left[\begin{array}{ccccccccccccc}
%1&0&0&0&0&0&0&0&0&0&0&0&0\\0&1&0&0&0&0&0&0&0&0&0&0&0\\0&0&1
%&0&0&0&0&0&0&0&0&0&0\\0&0&0&e^s&0&0&0&0&0&0&0&0&0
%\\0&0&0&0&e^{-s}&0&0&0&0&0&0&0&0\\0&0&0&0
%&0&e^{-s}&0&0&0&0&0&0&0\\0&0&0&0&0&0&e^{-s}&0&0&0&0&0&0
%\\0&0&0&0&0&0&0&1&0&0&0&0&0\\0&0&0
%&0&0&0&0&0&1&0&0&0&0\\0&0&0&0&0&0&0&0&0&1&0&0&0
%\\0&0&0&0&0&0&0&0&0&0&1&0&0\\0&0&0
%&0&0&0&0&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
%\end{array}\right],\nonumber \\[3mm]
%
%&&\hspace{-1cm}  \tiny \left[\begin{array}{ccccccccccccc}
%e^s&0&0&0&0&0&0&0&0&0&0&0&0
%\\0&e^s&0&0&0&0&0&0&0&0&0&0&0\\0&0&e^s&0
%&0&0&0&0&0&0&0&0&0\\0&0&0&1&0&0&0&0&0&0&0&0&0
%\\0&0&0&0&e^s&0&0&0&0&0&0&0&0\\0&0&0&0
%&0&e^s&0&0&0&0&0&0&0\\0&0&0&0&0&0&e^s&0&0&0&0&0&0
%\\0&0&0&0&0&0&0&1&0&0&0&0&0\\0&0&0
%&0&0&0&0&0&1&0&0&0&0\\0&0&0&0&0&0&0&0&0&1&0&0&0
%\\0&0&0&0&0&0&0&0&0&0&1&0&0\\0&0&0
%&0&0&0&0&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
%\end{array}\right],
%\nonumber \\[3mm]
%%s&-\sin s&0&0&0&0&0&0&0&0&0&0&0
%\\\sin s&\cos s&0&0&0&0&0&0&0&0&0&0&0\\0&0&1&0&0
%&0&0&0&0&0&0&0&0\\0&0&0&1&0&0&0&0&0&0&0&0&0
%\\0&0&0&0&\cos s&-\sin s&0&0&0&0&0&0&0\\0&0&0&0
%&\sin s&\cos s&0&0&0&0&0&0&0\\0&0&0&0&0&0&1&0&0&0&0&0&0
%\\0&0&0&0&0&0&0&1&0&0&0&0&0\\0&0&0
%&0&0&0&0&0&1&0&0&0&0\\0&0&0&0&0&0&0&0&0&1&0&0&0
%\\0&0&0&0&0&0&0&0&0&0&\cos s&\sin s&0\\0&0&0&0&0
%&0&0&0&0&0&-\sin s&\cos s&0\\0&0&0&0&0&0&0&0&0&0&0&0&1\end{array}
%\right],\nonumber \\[3mm]
%%
%&&\hspace{-1cm} \tiny \left[\begin{array}{ccccccccccccc}
%1&0&0&0&0&0&0&0&0&0&0&0&0
%\\0&\cos s&\sin s&0&0&0&0&0&0&0&0&0&0\\0&-\sin s&\cos s&0
%&0&0&0&0&0&0&0&0&0\\0&0&0&1&0&0&0&0&0&0&0&0&0
%\\0&0&0&0&1&0&0&0&0&0&0&0&0\\0&0&0
%&0&0&\cos s&\sin s&0&0&0&0&0&0\\0&0&0&0&0&-\sin s&\cos
%s&0&0&0&0&0&0
%\\0&0&0&0&0&0&0&1&0&0&0&0&0\\0&0&0
%&0&0&0&0&0&1&0&0&0&0\\0&0&0&0&0&0&0&0&0&\cos s&0&-\sin
%s&0\\0&0&0&0&0&0&0&0&0&0&1&0&0\\0&0&0 &0&0&0&0&0&0&\sin s&0&\cos
%s&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
%\end{array}\right],\nonumber \\[3mm]
%
&&\hspace{-1cm} \tiny \cdots, \left[\begin{array}{ccccccccccccc}
\cos s&0&\sin s&0&0&0&0&0&0&0&0&0&0
\\0&1&0&0&0&0&0&0&0&0&0&0&0\\-\sin s&0&\cos s
&0&0&0&0&0&0&0&0&0&0\\0&0&0&1&0&0&0&0&0&0&0&0&0
\\0&0&0&0&\cos s&0&\sin s&0&0&0&0&0&0\\0&0&0&0&0
&1&0&0&0&0&0&0&0\\0&0&0&0&-\sin s&0&\cos s&0&0&0&0&0&0
\\0&0&0&0&0&0&0&1&0&0&0&0&0\\0&0&0
&0&0&0&0&0&1&0&0&0&0\\0&0&0&0&0&0&0&0&0&\cos s&\sin s&0&0
\\0&0&0&0&0&0&0&0&0&-\sin s&\cos s&0&0\\0&0&0&0&0
&0&0&0&0&0&0&1&0\\0&0&0&0&0&0&0&0&0&0&0&0&1
\end{array}\right],\nonumber
%
 \ee
%
and $I_{13}$, respectively. Let $X=\sum_{i=1}^{13}a_iX_i$, then
%
\be && \hspace{-1cm} F(s_7.X_7)\circ F(s_6.X_6)\circ\cdots\circ
F(s_1.X_1)\;:\;X\;\mapsto\;\nonumber\\
&&(s_3a_{12}-s_2a_{10}-s_1a_9+a_1-s_5s_4a_8+s_5a_4-s_4a_5).X_1\nonumber\\
&&+(-s_6s_4a_8+s_3a_{11}-s_2a_9+s_1a_{10}+a_2+s_6a_4-s_4a_6).X_2\nonumber\\
&&+(-s_7s_4a_8-s_3a_9-s_2a_{11}-s_1a_{12}+a3+s_7a_4-s_4a_7).X_3\\
&&+(a_4-s_4a_8).X_4+(-s_6a_{10}-s_5a_9+s_5a_8+a_5+s_7a_{12}).X_5\nonumber\ee
\be
&&+(-s_6a_9+s_6a_8+s_5a_{10}+a_6+s_7a_{11}).X_6\nonumber\\
&&+(s_7a_8-s_6a_{11}-s_5a_{12}+a_7-s_7a_9).X_7+\sum_{i=1}^{13}a_i.X_i\nonumber
\ee
%
If $a_8$, and $a_9,a_8-2a_9\neq0$, then we can make the
coefficients of $X_1,\cdots,X_7$ vanish. Scaling $X$ if necessary,
we can assume that $a_8=1$. And $X$ is reduced to Case 1.\\
If $a_8=a_9\neq0$, and $a_{10}\neq0$, then we can make the
coefficients of $X_1\cdots,X_6$ vanish. Scaling $X$ if necessary,
we can assume that $a_8=1$. And $X$ is reduced to Case 2.\\
If $a_8=a_9\neq0$, $a_{10}=0$, and $a_{12}\neq0$, then we can make
the coefficients of $X_1,\cdots,X_5$, and $X_{10}$ vanish. Scaling
$X$ if necessary, we can assume that $a_8=1$. And $X$ is reduced
to Case 3.\\
If $a_8=a_9\neq0$, $a_{10}=a_{12}=0$, and $a_{11}\neq0$, then we
can make the coefficients of $X_1,\cdots,X_4$, $X_6$, $X_7$,
$X_{10}$, and $X_{12}$ vanish. Scaling $X$ if necessary, we can
assume that $a_8=1$. And $X$ is reduced to Case 4.\\
If $a_8=a_9\neq0$, $a_{10}=a_{11}=a_{12}=0$, then we can make the
coefficients of $X_1,\cdots,X_4$, and $X_{10},\cdots,X_{11}$
vanish. Scaling $X$ if necessary, we can assume that $a_8=1$. And
$X$ is reduced to Case 5.\\
If $a_8=0$, and $a_9\neq0$, then we can make the coefficients of
$X_1,\cdots,X_3,X_5,\cdots,X_8$ vanish. Scaling $X$ if necessary,
we can assume $a_9=1$. And $X$ is reduced to Case
6.\\
If $a_8\neq0$, $a_9=0$, and $a_{11}\neq0$, then we can make the
coefficients of $X_1,\cdots,X_3$, and $X_6$, $X_7$, and $X_9$
vanish. And $X$ is reduced to Case 7.\\
If $a_8\neq0$, $a_9=a_{11}=0$, and $a_{12}\neq0$, then we can make
the coefficients of $X_1,\cdots,X_3$, and $X_5$, $X_7$, $X_9$, and
$X_{11}$ vanish. And $X$ is reduced to Case 8.\\
If $a_8\neq0$, $a_9=a_{11}=a_{12}=0$, and $a_{10}\neq0$, then we
can make the coefficients of $X_1,\cdots,X_3$, and $X_5$, $X_6$,
$X_9$, and $X_{11}$ vanish. And $X$ is reduced to Case 9.\\
If $a_8\neq0$, and $a_9=a_{10}=a_{11}=a_{12}=0$, then we can make
the coefficients of $X_1,\cdots,X_3$, and $X_9,\cdots,X_{12}$
vanish. And $X$ is reduced to Case 10.\\
If $a_8=a_9=0$, $a_4\neq0$, and $a_{10}\neq0$, then we can make
the coefficients of $X_1,\cdots,X_3$, $X_5$, $X_6$, $X_8$, and
$X_9$ vanish. Scaling $X$ if necessary, we can assume that
$a_4=1$. And $X$ is reduced to Case 11.\\
If $a_4=a_8=a_9=0$, $a_{10}\neq0$, $a_{12}\neq0$, and
$a_6a_{12}+a_7a_{10}\neq a_5a_{11}$, then we can make the
coefficients of $X_1,\cdots,X_6$, $X_8$, and $X_9$ vanish. Scaling
$X$ if necessary, we can assume that $a_7=1$. And $X$ is reduced
to Case 12.\\
If $a_4=a_8=a_9=0$, $a_{10}\neq0$, $a_{12}\neq0$, and
$a_6a_{12}+a_7a_{10}=a_5a_{11}$, then we can make the coefficients
of $X_1$, $X_2$, and $X_4,\cdots,X_9$ vanish. And $X$ is reduced
to Case 13.\\
If $a_8=a_9=a_{10}=0$, and $a_4\neq0$, then we can make the
coefficients of $X_1,\cdots,X_3$, $X_5$, and $X_7,\cdots,X_{10}$
vanish. Scaling $X$ if necessary, we can assume that $a_4=1$. And
$X$ is reduced to Case 14.\\
If $a_8=\cdots=a_{10}=0$, $a_{12}=0$, $a_4\neq0$, and
$a_{11}\neq0$, then we can make the coefficients of
$X_1,\cdots,X_3$, and $X_8,\cdots,X_{10}$ vanish. Scaling $X$ if
necessary, we can assume that $a_4=1$. And $X$ is reduced to Case
15.\\
If $a_8=\cdots=a_{12}=0$, and $a_4\neq0$, then we can make the
coefficients of $X_1,\cdots,X_3$, and $X_8,\cdots,X_{10}$ vanish.
Scaling $X$ if necessary, we can assume that $a_4=1$. And $X$ is
reduced to Case 16.\\
If $a_4=a_8=a_9=a_{10}=0$, $a_{12}\neq0$, and $a_5a_{11}\neq
a_6a_{12}$, then we can make the coefficients of $X_1,\cdots,X_5$,
and $X_7,\cdots,X_{10}$ vanish. Scaling $X$ if necessary, we can
assume that $a_6=1$. And $X$ is reduced to Case 17.\\
If $a_4=a_8=a_9=a_{10}=0$, $a_{12}\neq0$, $a_5a_{11}=a_6a_{12}$,
and $a_6\neq0$, then we can make the coefficients of
$X_1,\cdots,X_5$, and $X_7,\cdots,X_{10}$ vanish. And $X$ is
reduced to Case 18.\\
If $a_4=a_6=a_8=a_9=a_{10}=0$, $a_{12}\neq0$,
$a_5a_{11}=a_6a_{12}$, and $a_6\neq0$, then we can make the
coefficients of $X_1,\cdots,X_5$, and $X_7,\cdots,X_{10}$ vanish.
And $X$ is reduced to Case 18.\\
If $a_4=a_6=a_8=\cdots=a_{11}=0$, $a_5a_{11}=a_6a_{12}$, and
$a_5,a_6,a_{12}\neq0$, then we can make the coefficients of $X_1$,
and $X_3,\cdots,X_{11}$ vanish.
And $X$ is reduced to Case 19.\\
If $a_4=a_8=a_9=a_{10}=a_{12}=0$, $a_5\neq0$, and $a_{11}\neq0$,
then we can make the coefficients of $X_1,\cdots,a_4$,
$X_6,\cdots,X_{10}$, and $a_12$ vanish. Scaling $X$ if necessary,
we can assume that $a_5=1$. And $X$ is reduced to Case 20.\\
If $a_4=a_8=\cdots=a_{12}=0$, and $a_5\neq0$, then we can make the
coefficients of $X_1$, $a_4$, and $X_8,\cdots,X_{12}$ vanish.
Scaling $X$ if necessary, we can assume that $a_5=1$. And $X$ is
reduced to Case 21.\\
If $a_4=a_5=a_8=a_9=a_{10}=a_{12}=0$, and $a_{11}\neq0$, then we
can make the coefficients of $X_2,\cdots,X_{10}$ and $a_{12}$
vanish. Scaling $X$ if necessary, we can assume that $a_{11}=1$.
And $X$ is reduced to Case 22.\\
If $a_4=a_5=a_8=\cdots=a_{12}=0$, and $a_6\neq0$, then we can make
the coefficients of $X_2$, $a_5$, and $X_7,\cdots,X_{12}$ vanish.
Scaling $X$ if necessary, we can assume that $a_6=1$. And $X$ is
reduced to Case 23.\\
If $a_4=a_5=a_6=0$, and $a_8=\cdots=a_{12}=0$, then we can make
the coefficients of $X_4,\cdots,X_{12}$ vanish. And $X$ is reduced
to Case 24.\\
If $a_4=a_8=a_9=a_{12}=0$, $a_{10}\neq0$, and $a_7a_{10}\neq
a_5a_{11}$, then we can make the coefficients of $X_1,\cdots,X_4$,
$X_6,\cdots,X_9$, and $a_{12}=0$ vanish. Scaling $X$ if necessary,
we can assume that $a_5=1$. And $X$ is reduced to Case 25.\\
If $a_4=a_8=a_9=a_{12}=0$, $a_7a_{10}=a_5a_{11}$, and
$a_{10}\neq0$, then we can make the coefficients of
$X_1,\cdots,X_4$, $X_6,\cdots,X_9$, and $a_{12}=0$ vanish. Scaling
$X$ if necessary, we can assume that $a_{10}=1$. And $X$ is
reduced to Case 26. And the Theorem follows. \hfill\ $\Box$

\medskip


According to our optimal system of one-dimensional subalgebras of
the full symmetry algebra $\bf g$, we need only find
group-invariant solutions for 26 one-parameter subgroups generated
by $X$ as Theorem 6. For example, as a direct consequence of
Theorem 3 and case 1 of Theorem 6, we deduce the following
conclusion:
%
\paragraph{Conclusion 2}
%
{\em Let $s,c_1,\cdots,c_6\in\RR$ with $c_1$, $c_2$, and
$c_6\neq0$, and $s$ be sufficiently small. Then, if
$u=U(t,x,y,z),\cdots, q=Q(t,x,y,z)$ be a solution of the system
(\ref{eq:1}), so are the functions
%
\begin{align*}
%
\tilde{u}=&c_1^sc_2^{-s}\big(\cos (c_3s)\cos (c_5s)-\sin
(c_3s)\sin (c_4s)\sin(c_5s)\big).U(\tilde{t},\tilde{x},\tilde{y},\tilde{z})\\
&-c_1^sc_2^{-s}\big(\sin (c_3s)\cos (c_5s)+\cos (c_3s)\sin
(c_4s)\cos(c_5s)\big).V(\tilde{t},\tilde{x},\tilde{y},\tilde{z})\\
&+c_1^sc_2^{-s}\cos (c_4s)\sin
(c_5s).W(\tilde{t},\tilde{x},\tilde{y},\tilde{z}), \\
\tilde{v}=&c_1^sc_2^{-s}\sin (c_3s)\cos
(c_4s).U(\tilde{t},\tilde{x},\tilde{y},\tilde{z})+c_1^sc_2^{-s}\cos (c_3s)\cos (c_4s).V(\tilde{t},\tilde{x},\tilde{y},\tilde{z})\\
&+c_1^sc_2^{-s}.\sin
(c_4s).W(\tilde{t},\tilde{x},\tilde{y},\tilde{z}),\qquad
\tilde{p}=c_6^{-s}.P(\tilde{t},\tilde{x},\tilde{y},\tilde{z}),\\
%
\tilde{w}=&-c_1^sc_2^{-s}\big(\cos (c_3s)\sin (c_5s)+\sin
(c_3s)\sin (c_4s)\cos
(c_5s)\big).U(\tilde{t},\tilde{x},\tilde{y},\tilde{z})\\
&+c_1^sc_2^{-s}\big(\sin (c_3s)\sin (c_5s)-\cos (c_3s)\sin
(c_4s)\cos
(c_5s)\big).V(\tilde{t},\tilde{x},\tilde{y},\tilde{z})\\
&+c_1^sc_2^{-s}\cos (c_4s)\cos
(c_5s).W(\tilde{t},\tilde{x},\tilde{y},\tilde{z}),\quad
\tilde{q}=c_1^{-2s}c_2^{2s}c_6^{-s}.Q(\tilde{t},\tilde{x},\tilde{y},\tilde{z}),
%
\end{align*}
%
where $\tilde{t}=c_1^s.t$, and
%
\begin{align*}
%
\tilde{x}=&c_2^s\big(\sin (c_5s)\sin (c_4s)\sin (c_3s)+\cos
(c_5s)\cos(c_3s)\big).x\\
&+c_2^s\big(\sin (c_3s)\cos (c_5s)-\cos (c_3s)\sin (c_4s)\sin
(c_5s) \big).y-c_2^s\cos (c_4s)\sin (c_5s).z,\\[2mm]
%
\tilde{y}=& -c_2^s\sin (c_3s)\cos (c_4s).x+(c_2s)\cos
(c_3s)\cos (c_4s).y-c_2^s\sin (c_4s).z,\\[2mm]
%
\tilde{z}=& c_2^s\big(\cos (c_3s)\sin (c_5s)-\sin (c_3s)\sin
(c_4s)\cos(c_5s)\big).x\\
&+c_2^s\big(\cos (c_3s)\sin (c_4s)\cos (c_5s)+\sin (c_3s)\sin
(c_5s)\big).y+c_2^s\cos (c_4s)\cos (c_5s).z.
%
\end{align*}}
%
The construction of the group-invariant solutions for each of the
one-dimensional subgroups in the optimal system proceeds in the
same fashion.
%
\section{Acknowledgements}
%
I am grateful to professor Ian M. Anderson for his consideration
and his mathematical career to the development the
"DifferentialGeometry" package of MAPLE 11. It is an applicable
tool to extremely complex and tedious geometrical computations.
%
\bebi
%
%\bibitem{BluKum} {\sc G.W. Bluman, S. Kumei}, {\em Symmetries and Differential Equations},
%Springer, New York, 1989.
%
\bibitem{Ibr} {\sc N.H. Ibragimov}, {\em Transformation Groups Applied to Mathematical Physics}, Reidel,
Dordrecht, 1985.
%
\bibitem{NadHej} {\sc M. M. Nadjafikhah} and {S.R. Hejazi}, {\em
}, To appear in Balkan Journal of Geometry and its Applications,
2009.
%
\bibitem{NadMeh} {\sc M. Nadjafikhah, A. Mahdipour-Shirayeh}, {\em
Galilean Classification of Spacetime Curves}, arXiv e-print:
arXiv:0711.1979.
%
\bibitem{OliSpe} {\sc F. Oliveri, M.P. Speciale}, {\em Exact solutions to the unsteady
equations of perfect gases through Lie group analysis and
substitution principles}, Int. J. Non-Linear Mech. 37 (2002)
257--274.
%
\bibitem{Olv2} {\sc P.J. Olver}, {\em Equivalence, Invariants,
and Symmetry}, Cambridge University Press, 1995.
%
\bibitem{Ovs} {\sc L.V. Ovsiannikov}, {\em Group Analysis of Differential Equations},
Academic Press, New York, 1982.
%
\bibitem{SekSha} {\sc T.R. Sekhar, V.D. Sharma}, {\em Similarity solutions for three dimensional Euler equations
using Lie group analysis}, Appl. Math. and Comp. 196 (2008)
147--157.
%
\bibitem{Ste} {\sc W.H. Steeb}, {\em Continuous symmetries, Lie algebras, differential
equations and computer algebra}, World Sci. Pub. Co., Singapore,
1996.
%
\bibitem{Udr} {\sc C. Udriste} and {\sc N. Bila}, {\em
Symmetry Lie Group of Monge-Ampere Equation}, Balkan Journal of
Geometry and its Applications 3, 2(1998), 121-133.



\eebi
%
\auas
Mehdi Nadjafikhah \\
School of Mathematics,\\
Iran University of Science and Technology,\\
Narmak-16, Theran, I.R.Iran.\\
E-mail:m\_nadjafikhah@iust.ac.ir
%
\end{document}

